What's New? Summarizing Contributions in Scientific Literature

With thousands of academic articles shared on a daily basis, it has become increasingly difficult to keep up with the latest scientific findings. To overcome this problem, we introduce a new task of disentangled paper summarization, which seeks to generate separate summaries for the paper contributions and the context of the work, making it easier to identify the key findings shared in articles. For this purpose, we extend the S2ORC corpus of academic articles, which spans a diverse set of domains ranging from economics to psychology, by adding disentangled "contribution" and "context" reference labels. Together with the dataset, we introduce and analyze three baseline approaches: 1) a unified model controlled by input code prefixes, 2) a model with separate generation heads specialized in generating the disentangled outputs, and 3) a training strategy that guides the model using additional supervision coming from inbound and outbound citations. We also propose a comprehensive automatic evaluation protocol which reports the relevance, novelty, and disentanglement of generated outputs. Through a human study involving expert annotators, we show that in 79%, of cases our new task is considered more helpful than traditional scientific paper summarization.

==> tables/cc_background_domain.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table}[]
\begin{tabular}{@{}lrrrrrrrrr@{}}
Metric                & R1    & R2    & R3    & R4    & R-L   & R-W   & R-S*  & R-SU  & BertScore \\
Biology               & 39.42 & 16.50 & 10.79 & 8.59  & 23.84 & 7.98  & 15.44 & 15.70 & 64.58     \\
Medicine              & 38.93 & 16.41 & 10.55 & 7.93  & 23.23 & 7.74  & 14.40 & 14.66 & 63.17     \\
Mathematics           & 39.14 & 14.61 & 7.92  & 5.15  & 22.53 & 8.79  & 14.29 & 14.67 & 61.78     \\
Computer science      & 40.15 & 13.86 & 7.55  & 5.15  & 21.80 & 7.80  & 15.17 & 15.49 & 62.12     \\
Unclassified          & 41.61 & 19.39 & 13.74 & 11.38 & 26.48 & 9.45  & 17.83 & 18.11 & 65.26     \\
Psychology            & 40.17 & 16.41 & 10.67 & 8.43  & 23.54 & 8.04  & 16.12 & 16.38 & 63.49     \\
Physics               & 40.60 & 16.10 & 9.44  & 6.97  & 23.99 & 9.13  & 16.35 & 16.70 & 62.97     \\
Chemistry             & 38.70 & 17.05 & 11.67 & 9.63  & 24.31 & 8.07  & 15.12 & 15.37 & 64.30     \\
Economics             & 39.07 & 13.73 & 7.83  & 5.70  & 21.92 & 7.94  & 14.86 & 15.16 & 60.89     \\
Materials science     & 39.93 & 17.32 & 11.83 & 9.80  & 24.89 & 8.78  & 17.07 & 17.34 & 64.48     \\
Geology               & 36.25 & 14.85 & 9.77  & 8.06  & 21.89 & 6.97  & 12.87 & 13.10 & 61.37     \\
Engineering           & 38.71 & 14.66 & 9.38  & 7.45  & 22.54 & 8.08  & 15.19 & 15.45 & 62.01     \\
Geography             & 44.32 & 23.77 & 18.84 & 16.98 & 30.44 & 10.90 & 21.36 & 21.61 & 65.69     \\
Environmental science & 44.13 & 23.94 & 19.44 & 17.91 & 30.58 & 11.39 & 21.88 & 22.11 & 65.98     \\
Business              & 40.62 & 16.75 & 11.23 & 9.09  & 24.57 & 8.95  & 16.92 & 17.20 & 62.02     \\
Sociology             & 38.79 & 14.47 & 9.23  & 7.31  & 22.83 & 8.04  & 15.28 & 15.56 & 60.28     \\
Political science     & 44.93 & 21.12 & 16.05 & 14.18 & 28.93 & 10.89 & 21.82 & 22.10 & 64.03     \\
Philosophy            & 36.21 & 18.22 & 14.53 & 13.64 & 26.93 & 9.80  & 15.91 & 16.17 & 58.38     \\
History               & 33.60 & 9.50  & 4.24  & 2.67  & 18.37 & 5.42  & 10.19 & 10.42 & 57.74
\end{tabular}
\caption{}
\label{tab:my-table}
\end{table}


==> tables/cc_contrib_domain.tex <==
\begin{table}[]
\begin{tabular}{@{}lrrrrrrrrr@{}}
Metric                & R1    & R2    & R3    & R4    & R-L   & R-W   & R-S*  & R-SU  & BertScore \\
Biology               & 38.35 & 16.14 & 10.60 & 8.46  & 24.61 & 9.93  & 15.33 & 15.74 & 64.23     \\
Medicine              & 32.35 & 12.49 & 7.85  & 6.04  & 20.99 & 9.19  & 10.83 & 11.31 & 61.75     \\
Mathematics           & 37.80 & 14.52 & 8.09  & 5.36  & 23.34 & 10.06 & 13.43 & 13.94 & 61.58     \\
Computer science      & 40.52 & 15.33 & 8.70  & 5.97  & 24.57 & 10.06 & 15.63 & 16.07 & 63.43     \\
Unclassified          & 38.27 & 17.35 & 12.18 & 10.10 & 25.79 & 11.09 & 15.92 & 16.35 & 64.00     \\
Psychology            & 37.26 & 14.78 & 9.52  & 7.59  & 23.39 & 9.72  & 14.41 & 14.84 & 62.95     \\
Physics               & 37.95 & 15.01 & 8.87  & 6.61  & 23.97 & 10.48 & 14.38 & 14.86 & 62.10     \\
Chemistry             & 38.33 & 16.94 & 11.68 & 9.72  & 25.23 & 9.96  & 15.53 & 15.93 & 63.93     \\
Economics             & 37.27 & 13.42 & 7.79  & 5.66  & 2.39 & 9.20  & 13.60 & 14.02 & 60.91     \\
Materials science     & 40.32 & 18.09 & 12.48 & 10.21 & 26.58 & 10.89 & 16.96 & 17.39 & 65.25     \\
Geology               & 36.20 & 14.66 & 9.52  & 7.81  & 22.39 & 8.37  & 13.50 & 13.84 & 61.16     \\
Engineering           & 37.73 & 15.57 & 10.23 & 8.09  & 24.66 & 10.77 & 14.84 & 15.28 & 62.15     \\
Geography             & 42.01 & 21.58 & 16.95 & 15.29 & 29.35 & 12.46 & 20.42 & 20.80 & 64.29     \\
Environmental science & 40.93 & 22.37 & 18.13 & 16.64 & 29.76 & 12.76 & 19.80 & 20.14 & 63.22     \\
Business              & 39.09 & 17.06 & 12.06 & 10.00 & 25.29 & 10.88 & 16.40 & 16.81 & 61.48     \\
Sociology             & 36.02 & 13.77 & 8.57  & 6.62  & 22.39 & 9.96  & 12.55 & 13.02 & 60.35     \\
Political science     & 39.85 & 18.83 & 14.17 & 12.60 & 27.59 & 12.43 & 17.49 & 17.91 & 62.31     \\
Philosophy            & 29.92 & 15.31 & 12.93 & 11.90 & 24.37 & 10.83 & 10.96 & 11.48 & 54.96     \\
History               & 37.07 & 14.01 & 7.84  & 3.95  & 25.48 & 10.26 & 12.40 & 12.75 & 66.57
\end{tabular}
\caption{}
\label{tab:my-table}
\end{table}


==> tables/disentanglement.tex <==
\begin{table}[htbp]
\centering
\begin{tabular}{@{}lrrrrrrrrr@{}}
\toprule
Model & R-1   & R-2   & R-3   & R-4   & R-L   & R-W   & R-S*  & R-SU  & BertScore \\\midrule
CC & 47.05 & 27.82 & 22.18 & 19.12 & 30.88 & 12.78 & 21.13 & 21.55 & 66.38 \\
MH & 49.11 & 30.49 & 25.11 & 22.20 & 34.03 & 14.55 & 23.86 & 24.27 & 67.49 \\\midrule
CC+MI & 49.15 & 30.08 & 23.80 & 20.16 & 32.28 & 13.30 & 22.18 & 22.63 & 67.92     \\
MH+MI & 47.11 & 29.74 & 25.19 & 22.78 & 33.57 & 14.37 & 22.36 & 22.77 & 66.60     \\\bottomrule
\end{tabular}
\caption{Disentanglement measures across different models. The lower values indicate more separation between the two mode outputs, thus better disentanglement.}
\label{tab:disentanglement}
\end{table}


==> tables/disentanglement_small.tex <==
\begin{table}[htbp]
\centering
\begin{tabular}{@{}lrrrrrrrr@{}}
\toprule
\multirow{2}{*}{Model} & \multicolumn{2}{c}{Novelty} & & \multicolumn{5}{c}{Disentanglement}\\\cmidrule{2-3}\cmidrule{5-9}
       & $N_1$ & $N_2$ & & D-1   & D-2   & D-3   & D-L   & DisBertScore \\\cmidrule{1-3}\cmidrule{5-9}
CC & 2.49 & 3.44 & & 52.95 & 72.18 & 77.82 & 69.12 & 33.62 \\
MH & 2.46 & 3.42 & & 50.89 & 69.51 & 74.89 & 65.97 & 32.51 \\\cmidrule{1-3}\cmidrule{5-9}
CC+INF & 2.47 & 3.44 & & 53.68 & 71.97 & 76.85 & 68.46 & 34.09 \\
MH+INF & 2.43 & 3.42 & & 53.35 & 71.47 & 76.16 & 67.20 & 33.86 \\\bottomrule
\end{tabular}
\caption{Novelty and Disentanglement measures across different models. For both measures, the higher values indicate better focus on the contributions (Novelty) and separation between the two mode outputs (Disentanglement), respectively.}
\label{tab:disentanglement}
\end{table}


==> tables/gold_eval_results_small.tex <==
\begin{table}[tbhp]
\centering
\begin{tabular}{@{}lrrrrr@{}}
\toprule
Metric               & R-1   & R-2   & R-3   & R-L   & BertScore \\\midrule
CC / Contrib & 39.37 & 15.86 & 9.70 & 24.73 & 63.28 \\
CC / Background & 30.59 & 11.22 & 7.20 & 19.08 & 55.76 \\
MH / Contrib & 38.63 & 15.53 & 9.51 & 24.68 & 62.84 \\
MH / Background & 29.82 & 10.61 & 6.64 & 18.51 & 55.24 \\\midrule
CC+INF / Contrib & 38.38 & 15.21 & 8.93 & 23.47 & 62.59 \\
CC+INF / Background & 30.14 & 11.10 & 7.26 & 19.00 & 55.55 \\
MH+INF / Contrib & 39.43 & 15.75 & 9.56 & 24.77 & 63.11 \\
MH+INF / Background & 29.14 & 10.25 & 6.39 & 18.48 & 54.92 \\\bottomrule
\end{tabular}
\caption{Relevance evaluation results on the test set. The higher indicates the better results.}
\label{tab:gold_results}
\end{table}


==> tables/mh_background_domain.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table}[]
\begin{tabular}{@{}lrrrrrrrrr@{}}
Metric                & R1    & R2    & R3    & R4    & R-L   & R-W   & R-S*  & R-SU  & BertScore \\
Biology               & 39.26 & 16.47 & 10.85 & 8.71  & 23.92 & 8.01  & 15.39 & 15.66 & 64.51     \\
Medicine              & 38.80 & 16.38 & 10.54 & 7.95  & 23.25 & 7.74  & 14.36 & 14.63 & 63.17     \\
Mathematics           & 38.79 & 14.65 & 8.03  & 5.26  & 22.86 & 8.83  & 14.05 & 14.46 & 61.82     \\
Computer science      & 40.24 & 14.23 & 7.86  & 5.39  & 22.25 & 7.91  & 15.27 & 15.59 & 62.41     \\
Unclassified          & 41.27 & 19.23 & 13.65 & 11.35 & 26.40 & 9.39  & 17.56 & 17.84 & 65.17     \\
Psychology            & 39.68 & 16.11 & 10.51 & 8.38  & 23.37 & 7.97  & 15.83 & 16.09 & 63.07     \\
Physics               & 40.67 & 16.54 & 9.83  & 7.31  & 24.67 & 9.29  & 16.36 & 16.73 & 63.50     \\
Chemistry             & 38.43 & 16.92 & 11.67 & 9.67  & 24.21 & 8.08  & 14.94 & 15.20 & 64.20     \\
Economics             & 39.22 & 14.02 & 8.09  & 5.82  & 22.20 & 8.04  & 14.89 & 15.20 & 61.31     \\
Materials science     & 40.30 & 17.78 & 12.28 & 10.15 & 25.37 & 8.98  & 17.44 & 17.71 & 64.80     \\
Geology               & 36.13 & 14.89 & 9.96  & 8.36  & 22.22 & 7.13  & 12.89 & 13.12 & 61.37     \\
Engineering           & 39.57 & 15.43 & 9.95  & 7.92  & 23.39 & 8.22  & 16.03 & 16.31 & 62.37     \\
Geography             & 43.57 & 23.44 & 19.09 & 17.39 & 30.35 & 10.93 & 20.87 & 21.12 & 65.59     \\
Environmental science & 44.24 & 24.19 & 19.55 & 18.05 & 30.75 & 11.44 & 22.15 & 22.38 & 66.03     \\
Business              & 41.18 & 17.37 & 11.59 & 9.22  & 24.77 & 9.08  & 17.18 & 17.46 & 62.74     \\
Sociology             & 38.50 & 14.01 & 8.69  & 6.81  & 21.84 & 7.70  & 14.51 & 14.79 & 60.38     \\
Political science     & 45.13 & 21.48 & 16.34 & 14.36 & 29.00 & 10.98 & 22.20 & 22.47 & 64.48     \\
Philosophy            & 34.63 & 17.52 & 14.43 & 13.75 & 25.92 & 9.52  & 15.04 & 15.29 & 57.69     \\
History               & 34.46 & 8.92  & 3.69  & 2.65  & 18.28 & 5.25  & 10.36 & 10.59 & 59.11
\end{tabular}
\caption{}
\label{tab:my-table}
\end{table}


==> tables/mh_contrib_domain.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table}[]
\begin{tabular}{@{}lrrrrrrrrr@{}}
Metric                & R1    & R2    & R3    & R4    & R-L   & R-W   & R-S*  & R-SU  & BertScore \\
Biology               & 38.46 & 16.25 & 10.71 & 8.57  & 24.81 & 10.00 & 15.48 & 15.89 & 64.13     \\
Medicine              & 32.34 & 12.38 & 7.79  & 6.01  & 20.74 & 9.12  & 10.87 & 11.33 & 61.27     \\
Mathematics           & 37.58 & 14.50 & 8.13  & 5.37  & 23.56 & 10.09 & 13.31 & 13.82 & 61.55     \\
Computer science      & 40.33 & 15.36 & 8.81  & 6.08  & 24.76 & 10.12 & 15.54 & 15.98 & 63.41     \\
Unclassified          & 38.57 & 17.71 & 12.48 & 10.36 & 26.07 & 11.20 & 16.25 & 16.68 & 64.02     \\
Psychology            & 37.38 & 14.82 & 9.63  & 7.71  & 23.42 & 9.80  & 14.64 & 15.05 & 62.47     \\
Physics               & 38.10 & 15.23 & 9.09  & 6.80  & 24.32 & 10.58 & 14.51 & 15.01 & 62.31     \\
Chemistry             & 37.91 & 16.51 & 11.35 & 9.46  & 24.87& 9.80  & 15.29 & 15.68 & 63.58     \\
Economics             & 37.04 & 13.57 & 7.97  & 5.82  & 22.29 & 9.30  & 13.42 & 13.83 & 60.74     \\
Materials science     & 40.28 & 18.18 & 12.46 & 10.07 & 26.69 & 10.84 & 17.21 & 17.63 & 65.38     \\
Geology               & 35.29 & 14.11 & 9.28  & 7.67  & 22.15 & 8.34  & 12.84 & 13.17 & 60.40     \\
Engineering           & 36.78 & 14.85 & 9.54  & 7.48  & 24.26 & 10.39 & 14.04 & 14.48 & 61.92     \\
Geography             & 42.17 & 22.04 & 17.60 & 15.92 & 29.93 & 12.79 & 20.86 & 21.23 & 64.67     \\
Environmental science & 41.81 & 23.32 & 19.12 & 17.60 & 30.59 & 13.18 & 21.26 & 21.61 & 63.54     \\
Business              & 38.25 & 16.05 & 11.15 & 9.02  & 24.31 & 10.59 & 15.11 & 15.50 & 60.75     \\
Sociology             & 36.65 & 14.77 & 9.65  & 7.74  & 24.06 & 10.76 & 14.05 & 14.47 & 60.90     \\
Political science     & 39.94 & 18.15 & 13.97 & 12.61 & 26.98 & 12.43 & 18.36 & 18.73 & 62.04     \\
Philosophy            & 37.99 & 21.33 & 18.76 & 17.94 & 28.99 & 13.41 & 22.85 & 23.29 & 58.22     \\
History               & 40.51 & 17.02 & 11.16 & 5.19  & 27.85 & 11.07 & 15.80 & 16.19 & 64.53
\end{tabular}
\caption{}
\label{tab:my-table}
\end{table}


==> tables/mh_contrib_domain_small.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table}[tbhp]
\centering
\begin{tabular}{@{}lrrrrr@{}}
\toprule
Metric                & R-1   & R-2   & R-3    & R-L    & BertScore \\\midrule
Biology               & 38.46 & 16.25 & 10.71  & 24.81  & 64.13     \\
Medicine              & 32.34 & 12.38 & 7.79   & 20.74  & 61.27     \\
Mathematics           & 37.58 & 14.50 & 8.13   & 23.56  & 61.55     \\
Computer science      & 40.33 & 15.36 & 8.81   & 24.76  & 63.41     \\
Unclassified          & 38.57 & 17.71 & 12.48  & 26.07  & 64.02     \\
Psychology            & 37.38 & 14.82 & 9.63   & 23.42  & 62.47     \\
Physics               & 38.10 & 15.23 & 9.09   & 24.32  & 62.31     \\
Chemistry             & 37.91 & 16.51 & 11.35  & 24.87  & 63.58     \\
Economics             & 37.04 & 13.57 & 7.97   & 22.29  & 60.74     \\
Materials science     & 40.28 & 18.18 & 12.46  & 26.69  & 65.38     \\\bottomrule
\end{tabular}
\caption{Automatic evaluation on contribution summarization for each of top-10 domains using \textsc{MultiHead} model.}
\label{tab:mh_dom}
\end{table}


==> tables/nouveau_rouge.tex <==
\begin{table}[tbhp]
\centering
\begin{tabular}{@{}lrr@{}}
\toprule
Model & $N_1$ & $N_2$ \\ \midrule
CC & 2.49 & 3.44 \\
MH & 2.46 & 3.42 \\
CC+MI & 2.45  & 3.32  \\
MH+MI & 2.39  & 3.33  \\ \bottomrule
\end{tabular}
\caption{Nouveau-ROUGE scores across models. The higher the score is, the better a model focuses only on describing contributions when asked to generate a contribution summary. \hh{statistical testing?}}
\label{tab:nouveau_rouge}
\end{table}


==> tables/results.tex <==
\begin{table}[tbhp]
\begin{tabular}{@{}lrrrrrrrrr@{}}
\toprule
Metric               & R-1   & R-2   & R-3   & R-4  & R-L   & R-W   & R-S*  & R-SU  & BertScore \\\midrule
CC / Contrib    & 39.16 & 15.96 & 10.11 & 7.86 & 24.65 & 10.25 & 15.66 & 16.12 & 63.22 \\
CC / Background & 41.84 & 17.24 & 10.94 & 8.45 & 24.55 & 8.43  & 17.00 & 17.29 & 63.78 \\
MH / Contrib    & 39.20 & 15.98 & 10.17 & 7.93 & 24.72 & 10.28 & 15.74 & 16.19 & 63.04 \\
MH / Background & 41.67 & 17.23 & 10.99 & 8.53 & 24.65 & 8.45  & 16.92 & 17.21 & 63.77 \\ \midrule
CC+MI / Contribution & 38.13 & 15.23 & 9.53  & 7.33 & 23.92 & 9.87  & 14.82 & 15.28 & 62.84 \\
CC+MI / Background   & 42.06 & 17.33 & 10.84 & 8.21 & 24.58 & 8.33  & 16.91 & 17.21 & 64.18 \\
MH+MI / Contribution & 37.98 & 15.40 & 9.86  & 7.73 & 24.15 & 10.01 & 14.87 & 15.32 & 62.25 \\
MH+MI / Background   & 40.86 & 16.55 & 10.54 & 8.21 & 24.00 & 8.23  & 16.27 & 16.56 & 63.09 \\ \bottomrule
\end{tabular}
\caption{Relevance evaluation results on the test set. The higher indicates the better results.}
\label{tab:results}
\end{table}

